Unification and Logarithmic Space

We present an algebraic characterization of the complexity classes Logspace and NLogspace, using an algebra with a composition law based on unification. This new bridge between unification and complexity classes is inspired from proof theory and more specifically linear logic and Geometry of Interaction. We show how unification can be used to build a model of computation by means of specific subalgebras associated to finite permutations groups. We then prove that whether an observation (the algebraic counterpart of a program) accepts a word can be decided within logarithmic space. We also show that the construction can naturally represent pointer machines, an intuitive way of understanding logarithmic space computing.

==> thm.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% STYLES

\newtheorem{theorm}{Theorem}[section]
\newtheorem{propositin}[theorm]{Proposition}
\newtheorem{definitin}[theorm]{Definition}
\newtheorem{lema}[theorm]{Lemma}
\newtheorem{corollay}[theorm]{Corollary}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% FONCTIONS


\newenvironment{leftbar2}
	{\def\FrameCommand{\hspace{12pt}\vrule width 2pt \hspace{7pt}}
		\MakeFramed {\advance\hsize-\width \FrameRestore}
	}
	{\endMakeFramed}

\newenvironment{leftbar1}
	{\def\FrameCommand{\hspace{10pt} \vrule width 0.6pt \hspace{7.7pt}}
		\MakeFramed {\advance\hsize-\width \FrameRestore}
	}
	{\endMakeFramed}

\newenvironment{leftbar11}
	{\def\FrameCommand{\hspace{10pt} \vrule width 0.6pt \hspace{-1.8pt} \vrule width 0.6pt \hspace{6.3pt}}
		\MakeFramed {\advance\hsize-\width \FrameRestore}
	}
	{\endMakeFramed}

\newenvironment{leftbar0}
	{\def\FrameCommand{\hspace{21pt}}
		\MakeFramed {\advance\hsize-\width \FrameRestore}
	}
	{\endMakeFramed}

\newcommand{\preuve}[1]{\proof{#1}}

\renewcommandx{\theorem}[2][1=~]{
\vbox{
	\begin{theorm}#1
		#2
	\end{theorm}
	}
}

\newcommandx{\theoreme}[2][1=~]{
\vbox{
	\begin{theorèe}#1
		#2
	\end{theorèe}
	}
}


\renewcommandx{\proposition}[2][1=~]{
\vbox{
	\begin{propositin}#1
		#2
	\end{propositin}
	}
}


\newcommandx{\define}[2][1=~]{
\vbox{
	\begin{definitin}#1
		#2
	\end{definitin}
	}
}

\renewcommandx{\definition}[2][1=~]{
\vbox{
	\begin{définitin}#1
		#2
	\end{définitin}
	}
}


\renewcommandx{\lemma}[2][1=~]{
\vbox{
	\begin{lema}#1
		#2
	\end{lema}
	}
}

\newcommandx{\lemme}[2][1=~]{
\vbox{
	\begin{leme}#1
		#2
	\end{leme}
	}
}


\renewcommandx{\corollary}[2][1=~]{
\vbox{
	\begin{corollay}#1
		#2
	\end{corollay}
	}
}

\newcommandx{\corollaire}[2][1=~]{
\vbox{
	\begin{corollaie}#1
		#2
	\end{corollaie}
	}
}

